On the role of depth predictions for 3D human pose estimation

Following the successful application of deep convolutional neural networks to 2d human pose estimation, the next logical problem to solve is 3d human pose estimation from monocular images. While previous solutions have shown some success, they do not fully utilize the depth information from the 2d inputs. With the goal of addressing this depth ambiguity, we build a system that takes 2d joint locations as input along with their estimated depth value and predicts their 3d positions in camera coordinates. Given the inherent noise and inaccuracy from estimating depth maps from monocular images, we perform an extensive statistical analysis showing that given this noise there is still a statistically significant correlation between the predicted depth values and the third coordinate of camera coordinates. We further explain how the state-of-the-art results we achieve on the H3.6M validation set are due to the additional input of depth. Notably, our results are produced on neural network that accepts a low dimensional input and be integrated into a real-time system. Furthermore, our system can be combined with an off-the-shelf 2d pose detector and a depth map predictor to perform 3d pose estimation in the wild.

==> OldBib.tex <==
\iffalse
\begin{thebibliography}{99}

\bibitem{LXSCLH14} Sijin Li and Antoni B Chan. 3d human pose estimation from monocular images with deep convolutional neural network. In ACCV, 2014

\bibitem{PZDD17} Georgios Pavlakos,  Xiaowei Zhou,  Konstantinos G Derpa-nis, and Kostas Daniilidis. \textit{Coarse-to-fine volumetric prediction for single-image 3d human pose}. In CVPR, 2017

\bibitem{SSLW17} Xiao Sun, Jiaxiang Shang, Shuang Liang, and Yichen Wei.  \textit{Compositional human pose regression}. In ICCV, 2017

\bibitem{SXWLW18} Xiao Sun, Bin Xiao, Fangyin Wei, Shuang Liang, and YichenWei. \textit{Integral human pose regression}. In ECCV, 2018

\bibitem{TKSLF16} Bugra Tekin, Isinsu Katircioglu, Mathieu Salzmann, Vincent Lepetit, and Pascal Fua.  \textit{Structured prediction of 3d human pose with deep neural networks}. BMVC, 2016

\bibitem{IPOS14} Catalin  Ionescu,  Dragos  Papava,  Vlad  Olaru,  and  Cristian Sminchisescu. Human3.6m: \textit{Large scale datasets and predictive methods for 3d human sensing in natural environments}. TPAMI, 2014

\bibitem{MHRL17} Julieta Martinez, Rayat Hossain, Javier Romero, and James J Little.  \textit{A simple yet effective baseline for 3d human pose estimation}. In ICCV, 2017

\bibitem{LS18} MegaDepth:  \textit{Learning Single-View Depth Prediction from Internet Photos}.  In Proc. Computer Vision and Pattern Recognition (CVPR), 2018

\bibitem{LDCTSLF19} Zhengqi Li, Tali Dekel, Forrester Cole, Richard Tucker, Noah Snavely, Ce Liu, and William T. \textit{Freeman Learning the Depths of Moving People by Watching Frozen People}. In Proc. Computer Vision and Pattern Recognition (CVPR), 2019

\bibitem{CL17} Ju Yong Change and Kyoung Mu Lee. \textit{2d-3d pose consistency-based conditional random fields for 3d human pose estimation}. CVIU, 2018

\bibitem{CR17} Ching-Hang Chen and Deva Ramanan. \textit{3d human pose estimation=2d pose estimation+matching}. In CVPR, 2017

\bibitem{FXWLZ18} Hao-Shu Fang, Yuanlu Xu, Wenguan Wang, Xiaobai Liu, and Song-Chun Zhu. Learning pose grammar to encode human body configuration for 3d pose estimation. In AAAI, 2018

\bibitem{PHK16} Sungheon Park, Jihye Hwang, and Nojun Kwak. 3d human pose estimation using convolutional neural networks with 2d pose information. In ECCV, 2016

\bibitem{YOWRLW18} Wei Yang, Wanli Ouyang, Xiaolong Wang, Jimmy Ren, Hongsheng Li, and Xiaogang Wang. 3d human pose estimation in the wild by adversarial learning. In CVPR, 2018.

\bibitem{MCL19} Gyeongsik Moon, Ju Yong Chang, and Kyoung Mu Lee. Camera Distance-aware Top-down Approach for 3d multi-person Pose Estimation from a Single RGB Image. In ICCV , 2019.

\bibitem{RWS17} Gregory Rogez, Philippe Weinzaepfel, and Cordelia Schmid. Ler-net: Localization-classification-regression for human pose. In CVPR, 2017.

\bibitem{RWS2019} Gregory Rogez, Philippe Weinzaepfel, and Cordelia Schmid. Ler-net++: Multi-person 2d and 3d pose detection in natural images. IEE TPAMI, 2019.

\bibitem{MRCFSXT17} Dushyant Mehta, Helge Rhodin, Dan Casas, Pascal Fua, Oleksandr Sotnychenko, Weipeng Xu, and Christian Theobalt. Monocular 3d human pose estimation in the wild using improved cnn supervision. In 3dV, 2017.

\bibitem{MSMXSMT18} Dushyant Mehta, Oleksandr Sotnychenko, Franziska Mueller, Weipeng Xu, Srinath Sridhar, Gerard Pons-Moll, and Christian Tehobalt. Single-shot multi-person 3d pose estimation from monocular rgb. In 3dV, 2018. 

\bibitem{ZHSXW17} Xingyi Zhou, Qixing Huang, Xiao Sun, Xiangyang Xue, and Yichen Wei.  Weakly supervised transfer for 3d human pose estimation in the wild. In ICCV, 2017

\bibitem{GKCR16} Ravi Garg, Vijay Kumar B G, Gustavo Carneiro, and Ian Reid. Unsupervised CNN for Single View Depth Estimation: Geometry to the Rescue. In ECCV, 2016

\bibitem{BK01} C. Barron and I. A. Kakadiaris. Estimating anthropometry and pose from a single uncalibrated image. CVIU, 2001. 

\bibitem{BKLGRB16} F. Bogo,  A. Kanazawa,  C. Lassner,  P. Gehler,  J. Romero, and M.J. Black. Keep it SMPL: Automatic estimation of 3d human pose and shape from a single image. In ECCV, 2016.

\bibitem{PC04} V. Parameswaran and R. Chellappa.  View independent human body pose estimation from a single perspective image. In CVPR, 2004.

\bibitem{ZSZLW16}  X. Zhou,  X. Sun,  W. Zhang,  S. Liang,  and Y. Wei.   Deep kinematic pose regression. In ECCV Workshops, 2016.

\bibitem{YIKWG16} Hashim Yasin, Umar Iqbal, Bjorn Kruger, Andreas Weber,and Juergen Gall.  A dual-source approach for 3d pose estimation from a single image. In CVPR, 2016.

\bibitem{TRA17} Denis Tome,  Chris Russell,  and Lourdes Agapito.   Lifting from the deep: Convolutional 3d pose estimation from a sin-gle image. In CVPR, 2017.

\bibitem{M17} Francesc Moreno-Noguer. 3d human pose estimation from a single image via distance matrix regression. In CVPR, 2017.

\bibitem{ZZPLDD19} Xiaowei  Zhou,  Menglong  Zhu,  Georgios  Pavlakos,  Spyri-don Leonardos, Konstantinos G Derpanis, and Kostas Daniilidis.  Monocap:  Monocular human motion capture using a cnn coupled with a geometric prior. TPAMI, 2019

\bibitem{JY17} Ehsan Jahangiri and Alan L Yuille.  Generating multiple diverse hypotheses for human 3d pose consistent with 2d joint detections. In ICCV, 2017

\bibitem{PML16} B. Peng, S. Mall, and Z Luo. \textit{Multi-View 3 D Pose Estimation from Single Depth Images} arXiv:2004.03989v1 2016. 

\bibitem{M-JR-RM-SM-C18} Manuel J. Marin-Jimenez, Francisco J. Romero-Ramirez, Rafael Muñoz-Salinas, Rafael Medina-Carnicer. \textit{3d human pose estimation from depth maps using a deep combination of poses}. Journal of Visual Communication and Image Representation, 2018

\bibitem{VL20}  Márton Véges and András Lőrincz. \textit{Multi-person Absolute 3d Human Pose Estimation with Weak Depth Supervision}. In ICAAN, 2020.

\bibitem{SW65} S. S. Shapiro, M. B. Wilk \textit{An Analysis of Variance Test for Normality (Complete Samples)}. In Biometrika , Vol. 52, No. 3/4. (Dec., 1965), pp. 591-611.

\bibitem{D52} Anderson TW, Darling DA \textit{Asymptotic theory of certain ‘goodness-of-fit’ criteria based on stochastic processes}. Ann Math Stat 23:193–212 (1952)

\bibitem{D70} R. D’Agostino. \textit{Transformation to normality of the null distribution of g1}. Biometrika. 57 (3): 679–681 (1970)

\bibitem{SHKF12} N. Silberman, D. Hoiem, P. Kohli, R. Fergus \textit{Indoor Segmentation and Support Inferencefrom RGBD Images}. In ECCV 2012

\bibitem{GB10} X. Glorot, Y. Bengio \textit{Understanding the difficulty of training deep feedforward neural networks}. In Proceedings of the Thirteenth International Conference on Artificial Intelligence and Statistics, JMLR Workshop and Conference Proceedings 9:249-256, 2010

\bibitem{TF15}     M. Abadi and
    A. Agarwal and
    P. Barham and
    E. Brevdo and
    Z. Chen and
    C. Citro and
    G. Corrado and
    A. Davis and
    J. Dean and
    M. Devin and
    S. Ghemawat and
    I. Goodfellow and
    A. Harp and
    G. Irving and
    M. Isard and
    Y. Jia and
    R. Jozefowicz and
    L. Kaiser and
    M. Kudlur and
    J. Levenberg and
    D. Man\'{e} and
    R. Monga and
    S. Moore and
    D. Murray and
    C. Olah and
    M. Schuster and
    J. Shlens and
    B. Steiner and
    I. Sutskever and
    K. Talwar and
    P. Tucker and
    V. Vanhoucke and
    V. Vasudevan and
    F. Vi\'{e}gas and
    O. Vinyals and
    P. Warden and
    M. Wattenberg and
    M. Wicke and
    Y. Yu and
    X. Zheng.
    \textit{Tensorflow,  Large-Scale Machine Learning on Heterogeneous Systems}, http://tensorflow.org/ 2015
    
    
\bibitem{ZC15}  Li,  S., Zhang, W., Chan, A.B.: \textit{Maximum-margin structured learning with deepnetworks for 3d human pose estimation}. In: Proceedings of the IEEE internationalconference on computer vision. pp. 2848–2856 (2015)

\bibitem{CH-MSWS19} Z. Cao and G. Hidalgo Martinez and T. Simon and S. Wei and Y. A. Sheikh
\textit{OpenPose: Realtime Multi-Person 2d Pose Estimation using Part Affinity Fields}. In IEEE Transactions on Pattern Analysis and Machine Intelligence (2019)

\bibitem{WRKS16} S.Wei, V. Ramakrishna, T. Kanade, Y. Sheikh \textit{Convolutional Pose Machines}. In CVPR 2016

\end{thebibliography}
\fi
